Towards an integrated modeling of the plasma-solid interface

Solids facing a plasma are a common situation in many astrophysical systems and laboratory setups. Moreover, many plasma technology applications rely on the control of the plasma-surface interaction. However, presently often a fundamental understanding of them is missing, so most technological applications are being developed via trial and error. In the majority of plasma simulations surface processes are either neglected or treated via phenomenological parameters such as sticking coefficients, sputter rates or secondary electron emission coefficients. However, those parameters are known only in some cases and with very limited accuracy. Similarly, while surface physics simulations have often studied the impact of single ions or neutrals, so far, the influence of a plasma medium and correlations between successive impacts have not been taken into account. Such an approach cannot have predictive power. In this paper we discuss in some detail the physical processes a the plasma-solid interface which brings us to the necessity of coupled plasma-solid simulations. We briefly summarize relevant theoretical methods from solid state and surface physics that are suitable to contribute to such an approach and identify four methods. The first are mesoscopic simulations such as kinetic Monte Carlo (KMC) and molecular dynamics (MD) that are able to treat complex processes on large scales but neglect electronic effects. The second are quantum kinetic methods based on the quantum Boltzmann equation that give access to a more accurate treatment of surface processes using simplifying models for the solid. The third approach are ab initio simulations of surface process that are based on density functional theory (DFT) and time-dependent DFT. The fourths are nonequilibrium Green functions that able to treat correlation effects in the material and at the interface.

==> references.tex <==
 
\section*{References}
\begin{thebibliography}{60}

%\bibitem{doe-report-17} Skiff F and Wurtele J (eds.) 2017 \textit{Report of the panel on Frontiers of Plasma Science}, U.S. Department of Energy

%\bibitem{plasma-road-map-17} Adamovich I, Baalrud S D, Bogaerts A, Bruggeman P J, Cappelli M, Colombo V, Czarnetzki U, Ebert U, Eden J G, Favia P \textit{et al.}  2017 
%{\it J.~Phys.~D:~Applied Physics} \textbf{50}, 323001
 
%\bibitem{hagelaar_2005} Hagelaar G J M and  Pitchford  C 2005, Plasma Sources Sci. Technol. \textbf{14}, 722

%\bibitem{donko_2016} Donko Z and Dyatko N 2016, Eur. Phys. J. D \textbf{70}, 135

%\bibitem{ebert_2016} Teunissen J and Ebert U 2016, 
%Plasma Sources Sci. Technol. \textbf{25}, 044005

%\bibitem{becker_2017} Becker MM, Kählert H, Sun A, Bonitz M, and Loffhagen D 2017, Plasma Sources Sci. Technol. \textbf{26}, 044001

%\bibitem{derszi_2015}  Derzsi A, Korolov I, Schüngel E, Donko, Z and Schulze J 2015,  Plasma Sources Sci. Technol. \textbf{24}, 034002

%\bibitem{phelps_1999} Phelps A V and Petrovic Z L 1999,  Plasma Sources Sci. Technol. \textbf{8}, R21

%\bibitem{michely} Michely

%\bibitem{brault_frontiers_18} Brault P 2018,
%Multiscale Molecular Dynamics simulation of plasma processing: Application to plasma sputtering,
%Frontiers Phys., in press.

%\bibitem{zhao_prb_15} Zhao S, Kang W, Xue J, Zhang X, and Zhang P 2015 
%Comparison of electronic energy loss in graphene and BN sheet by means of time-dependent density functional theory
%J. Phys.: Cond. Matt. \textbf{27} (2), 025401

%\bibitem{balzer_prb_16} Balzer K, Schlünzen N, and Bonitz M 2016
%Stopping dynamics of ions passing through correlated honeycomb clusters
%\textit{Phys. Rev. B} \textbf{94}, 245118

%\bibitem{interface} This concept is based on a research project devoted to plasma-surface physics that is being developed at Kiel University and was first presented by M. Bonitz at the Conference \textit{Quo vadis--complex plasmas}, Hamburg, August 2015, and at the \textit{GEC} in Bochum, October 2015.

%\bibitem{li_2013} Li Y and Go D B 2013, J. Appl. Phys. \textbf{103}, 234104

%\bibitem{campanell_2016} Campanell M D and Umansky M V 2016, Phys. Rev. Lett. \textbf{116}, 085003

%\bibitem{sheehan_2013} Sheehan J P, Hershkowitz N, Kaganovich I D, Wang H, Raitses Y, Barnat E V, Weatherford B R, and Sydorenko D, 
%Phys. Rev. Lett. \textbf{111}, 075002

%\bibitem{bronold_prl15} Bronold F X and Fehske H 2015 {\it Phys. Rev. Lett.} 
%\textbf{115}, 225001
%Absorption of an electron by a dielectric wall,

%\bibitem{pamperin_prb15} Pamperin M, Bronold F X and Fehske H 2015  
%Many-body theory of the neutralization of strontium ions on a gold surface, 
%{\it Phys. Rev. B} \textbf{91}, 035440

%\bibitem{bronold_epjd_18} Bronold F X, Fehske H, Pamperin M, and Thiessen E 2018  
%Electron kinetics at the plasma interface
%{\it Eur. Phys. J. D} \textbf{72}:88

%\bibitem{sun_psst_2018} Sun A, Becker M M, Loffhagen D 2018, 
%PIC/MCC simulation of capacitively coupled discharges in helium: boundary effects
%Plasma Sources Sci. Technol., in press

%\bibitem{bonitz_psst18} Bonitz M, Filinov A, Abraham J W, and Loffhagen D, Plasma Sources Sci. Technol., accepted for publication, arXiv:1802.08710

% review on ab initio TDDFT simulation and some models
%\bibitem{brenig-pehlke_08} Brenig W and Pehlke E 2008 {\it Progress in Surface 
%Science} \textbf{83}, 263
%Reaction dynamics of H2 on Si. Ab initio supported model calculations,

%\bibitem{schluenzen_cpp_16} Schl\"unzen N and Bonitz M 2016
%\textit{Contrib. Plasma Phys.} \textbf{56} (1) 5

%\bibitem{marini} Marini A,  Hogan C, Grüning M, and Varsano D 2009, 
%“Yambo: an ab initio tool for excited state calculations”,
%Comp. Phys. Comm. \textbf{180}, 1392 

%\bibitem{hutter_12} Hutter J 2012
%WIREs Comput. Mol. Sci. \textbf{2}, 604 

%\bibitem{gross-book} Gross A, \textit{Theoretical Surface Science}, 2nd ed., 
%Springer 2009.

%\bibitem{ott_prl_11} Ott T and Bonitz M 2011
%Diffusion in a strongly coupled magnetized plasma
%\textit{Phys. Rev. Lett.} \textbf{107}, 135003 

%\bibitem{com-plasmas_14}
%\textit{Complex Plasmas: Scientific Challenges and Technological Opportunities}, 
%Bonitz M, Lopez J, Becker K, and Thomsen H (eds.), Springer 2014.

%\bibitem{nakano_08} Nakano A \textit{et al.} 2008 
%De Novo Ultrascale atomistic simulations on high-end parallel supercomputers
%International Journal of High-Performance Computing Applications \textbf{22}, 
%113

%\bibitem{piana_13} Piana S, Lindorff-Larsena K, and Shawa D E 2013 \textit{Proc. 
%Nat. Acad. Sciences} \textbf{110}, 5915
%Atomic-level description of ubiquitin folding

%\bibitem{voter_97} Voter A F 1997
%\textit{Phys. Rev. Lett.} \textbf{78}, 3908

%\bibitem{parrinello_pnas_02}
%Laio A and Parrinello M 2002 {\em Proc. Natl. Acad. Sci. U.S.A.\/} {\bf 99}
%  12562--12566 
  %ISSN 0027-8424 

%\bibitem{Sorensen2000}
%S{\o}rensen M~R and Voter A~F 2000 {\em J. Chem. Phys.\/} {\bf 112} 9599%--9606

%\bibitem{Bal2015}
%Bal K~M and Neyts E~C 2015 {\em J. Chem. Theory Comput.\/} {\bf 11} 4545%--4554

%\bibitem{abraham_jap_16} Abraham J W, Strunskus T, Faupel F, and Bonitz M 2016
%Molecular dynamics simulation of gold cluster growth during sputter deposition
%\textit{J. Appl. Phys.} \textbf{119}, 185301.

%\bibitem{abraham_cpp_18} Abraham J W and Bonitz M 2018
%Molecular dynamics simulation of Ag-Cu cluster growth on a thin polymer film,
%\textit{Contrib. Plasma Phys.} \textbf{58}, 164 

%\bibitem{filinov_psst18_1} Filinov A, Bonitz M, and Loffhagen D 2018, Plasma Sources Sci. Technol. \textbf{27}, 064003 (2018),
%arXiv:1802.03466

% pehlke diffusion

%\bibitem{franke_prb_10} Franke A and Pehlke E 2010 
% Diffusion of 1,4-butanedithiol on Au(100)-1x1): A DFT-based master-equation approach
%\textit{Phys. Rev. B} \textbf{82}, 205423

%\bibitem{neyts2017molecular}
%Neyts E~C and Brault P 2017 {\em Plasma Process. Polym.\/} {\bf 14} ISSN
%  1612-8869 

%\bibitem{Neyts2012mdmc}
%Neyts E~C and Bogaerts A 2012 {\em Theor. %Chem. Acc.\/} {\bf 132} 1320


%\bibitem{Perez2009_voter}
%Perez D, Uberuaga B~P, Shim Y, Amar J~G and Voter A~F 2009 {\em Chapter 4
%  Accelerated Molecular Dynamics Methods: Introduction and Recent
%  Developments\/} ({\em Annu. Rep. Comput. Chem.\/} vol~5) ed Wheeler R~A
%  (Elsevier, Amsterdam) pp 79 -- 98

%\bibitem{Voter2002}
%Voter A~F, Montalenti F and Germann T~C 2002 {\em Annu. Rev. Mater. Sci.\/}
%  {\bf 32} 321%--346

%\bibitem{abraham_epjd_17} Abraham J W, Hinz A, Strunskus T, Faupel F, and Bonitz 
%M 2018
%Formation of polymer-based nanoparticles and nanocomposites by plasma-induced 
%deposition methods,
%\textit{Eur. Phys. J. D} 72:92 (2018)

%metadynamics

%\bibitem{laio_ropp_08}
%Laio A and Gervasio F~L 2008 {\em Rep. Prog. Phys.\/} {\bf 71} 126601
%Escaping free-energy minima

%\bibitem{bonitz_qkt} Bonitz M, \textit{Quantum Kinetic Theory}, 2nd ed., 
%Springer 2016.

%\bibitem{bonitz_pla_16} Bonitz M 1996
%Correlation time approximation in kinetic theory
%\textit{Phys. Lett. A} \textbf{221}, 85 

% KMC, MD, accelerated MD
%\bibitem{bonitz_cpp_12} Bonitz M, Rosenthal L, Fujioka K, Zaporojtchenko V, 
%Faupel F, and Kersten H 2012
%Towards a particle based simulation of complex plasma driven nanocomposite 
%formation
%{\it Contrib. Plasma Phys.} \textbf{52} (10), 890-898.


%\bibitem{filinov_psst18_2} Filinov A, Bonitz M, and Loffhagen D 2018 Plasma Sources Sci. Technol. \textbf{27}, 064002 (2018), 
%arXiv:1802.01985

%\bibitem{bonitz_pla_96} Bonitz M and Kremp D 1996 {\it Phys. Lett. A} 
%\textbf{212}, 83

%Rate equation model
%\bibitem{brenig_zpb79} Brenig W 1979 {\it Z. Phys. B - Condensed Matter} {\bf 36}, 81
%\bibitem{mc2} Böheim J and Brenig W 1979 {\it Z. Phys. B Condensed Matter} {\bf 
%41}, 243

%\bibitem{k1} Müller H and Brening W 1979 {\it Z. Phys. B - Condensed Matter} 
%{\bf 34}, 165

%\bibitem{k2} Leuthäusser U 1981 {\it Z. Phys. B - Condensed Matter} {\bf 44}, 
%101


%\bibitem{s1} Brako R and Newns D M 1982 {\it Phys. Rev. Lett.} \textbf{48}, 
%1859; Brako R 1982 {\it Surf. Sci.} {\bf 123} 439


%-----------

% transition state theory
%\bibitem{vineyard_57} G H Vineyard 1957 
%Frequency factors and isotope effects in solid state rate processes
%\textit{J. Phys. Chem. Solids} \textbf{3}, 121

% NEB
%\bibitem{mills_prl_94} Mill G and Jönsson H 1994
%
%\textit{Phys. Rev. Lett.} \textbf{72}, 1124

% NEB improbed
%\bibitem{henkelmann_jcp_00} Henkelman G and Jönsson H 2000 
% Improved tangent estimate in the nudged elastic band method for finding 
%minimum energy paths and saddle points
%\textit{J. Chem. Phys.} \textbf{113}, 9978


%\bibitem{maranzana_pccp_07} Maranzana A, Barker J R, and Tonachini G 2007
%Master equation simulations of competing unimolecular and bimolecular 
%reactions: application to OH production in the reaction of acetyl radical with O2
%\textit{Phys. Chem. Chem. Phys.} \textbf{9}, 4129

%\bibitem{robertson_pccp_07} Robertson S H, Pilling M J, Jitariu L C, and Hillier 
%I H 2007
%Master equation simulations of competing unimolecular and bimolecular reactions: application to OH production in the reaction of acetyl radical with O2
%\textit{Phys. Chem. Chem. Phys.} \textbf{9}, 4085

% hyperdynamics and so on

%\bibitem{voter_98} Voter A F and Germann T C 1998
%\textit{Mater. Res. Soc. Symp. Proc.} \textbf{528}, 221

%\bibitem{neyts} Neyts


%\bibitem{Voter1997}
%Voter A~F 1997 {\em Phys. Rev. Lett.\/} {\bf 78}(20) 3908%--3911

%\bibitem{Marcelin1915_tst}
%Marcelin R 1915 {\em Ann. Phys.\/} {\bf 3} 120

%\bibitem{Eyring1935_TST}
%Eyring H 1935 {\em J. Chem. Phys.\/} {\bf 3} 107%--115

%\bibitem{Fichthorn2009}
%Fichthorn K~A, Miron R~A, Wang Y and Tiwary Y 2009 {\em J. Phys. Condens.
%  Matter\/} {\bf 21} 084212

%\bibitem{Miron2003bondboost}
%Miron R~A and Fichthorn K~A 2003 {\em J. Chem. Phys.\/} {\bf 119} 6210%--6216

%\bibitem{Bal2016fuel}
%Bal K~M and Neyts E~C 2016 {\em Chem. Sci.\/} {\bf 7} 5280--5286

%\bibitem{Georgieva2011tad}
%Georgieva V, Voter A~F and Bogaerts A 2011 {\em Cryst. Growth Des.\/} {\bf 11}
%  2553%--2558 

%\bibitem{Voter1998}
%Voter A~F 1998 {\em Phys. Rev. B\/} {\bf 57}(22) R13985%--R13988

%\bibitem{Perez2015parrep}
%Perez D, Uberuaga B~P and Voter A~F 2015 {\em Comput. Mater. Sci.\/} {\bf 100}  90--103 

%\bibitem{Uberuaga2003ex_parrep}
%Uberuaga B~P, Voter A~F, Sieber K~K and Sholl D~S 2003 {\em Phys. Rev. Lett.\/}
%  {\bf 91}(10) 105901


%\bibitem{Duan2005ex_parrep}
%Duan Y, Halley J~W, Curtiss L and Redfern P 2005 {\em J. Chem. Phys.\/} {\bf
%  122} 054702 \

%\bibitem{Warner2007ex_parrep}
%Warner D~H, Curtin W~A and Qu S 2007 {\em Nat. Mater.\/} {\bf 6} 876%--881

%\bibitem{abraham_diss_18} Abraham J W 2018,  \textit{Formation of Metal-Polymer Nanocomposites by Plasma-Based Deposition Methods: Kinetic Monte Carlo and Molecular Dynamics Simulations}, PhD dissertation, Kiel University

%\bibitem{Schwartzkopf2015}
%Schwartzkopf M, Santoro G, Brett C~J, Rothkirch A, Polonskyi O, Hinz A,
%  Metwalli E, Yao Y, Strunskus T, Faupel F, M\"{u}ller-Buschbaum P and Roth S~V
%  2015 {\em ACS Appl. Mater. Interfaces\/} {\bf 7} 13547
  %--13556


% Selective Process a

%\bibitem{nose} Nose S 1984 
% A unified formulation of the constant temperature molecular dynamics method
%\textit{J. Chem. Phys.} \textbf{81}, 511

%\bibitem{klimontovich_sp} Klimontovich Yu L 1986
%\textit{Statistical Physics} Harwood Academic Publishers 

%\bibitem{bonitz_un} Bonitz M, \textit{Lectures on plasma theory}, unpublished.

%\bibitem{lacroix_prb_14} Lacroix D, Hermanns S, Hinz C, and Bonitz M 2014
%Ultrafast dynamics of finite Hubbard clusters - a stochastic mean field approach
%\textit{Phys. Rev. B} \textbf{90}, 125112

%functional hypothesis
%\bibitem{bogoljubov} Bogolyubov N N \textit{Problems of Dynamic Theory in 
%Statistical Physics.} Gostekhizdat, Moscow-Leningrad 1946 (in Russian). 

%\bibitem{bgk-integral}  Bhatnagar P L, Gross E P, and Krook M 1954 
%A Model for Collision Processes in Gases. I. Small Amplitude Processes in 
%Charged and Neutral One-Component Systems. 
%Phys. Rev. \textbf{94} (3): 511–525

%\bibitem{abraham_jap_15} Abraham J W,  Kongsuwan N, Strunskus T, Faupel F, and  
%Bonitz M 2015,
%Simulation of Nanocolumn Formation in a Plasma Environment
%\textit{J. Appl. Phys.} \textbf{117}, 014305 

%\bibitem{boening_prl_08} Böning J, Filinov A, Ludwig P, Baumgartner H, Bonitz M, 
%and  Lozovik Yu E 2008,
%Melting of trapped few particle systems
%\textit{Phys. Rev. Lett.} \textbf{100}, 113401 

%\bibitem{comment_exactness} This means we consider here only models that have 
%this property.

% experiments on Ar on Pt(111) 
%\bibitem{expPt} Mullins C B, Rettner C T, Auerbach D J, and Weinberg W H 1989 {\it Chem. Phys. Lett.} {\bf 163}, 111

%\bibitem{michta_cpp15} Michta D, Graziani F, and Bonitz M 2015 \textit{Contrib. Plasma Phys.} \textbf{55}, 437

%\bibitem{zhandos_pop18} Moldabekov Z, Bonitz M, and Ramazanov T 2018, \textit{Phys. Plasmas} \textbf{25}, 031903

%\bibitem{balzer_lnp_13} \textit{Nonequilibrium Green's Functions Approach to Inhomogeneous Systems},
%Balzer K and Bonitz M, Springer 2013

%MD
%\bibitem{graves_jpd_09} Graves D B and Brault P 2009, 
%Molecular dynamics for low temperature plasma-surface interaction studies,
%J. Phys. D: Appl. Phys. \textbf{42} 194011

%\bibitem{helmholtz} H. Helmholtz 1853, Ann. Phys. (Berlin) \textbf{165}, 211 

%\bibitem{heinisch_2012_electron} R. L. Heinisch,
%F. X. Bronold, and H. Fehske, 
%\textit{Electron surface layer at the interface of a plasma and a dielectric wall}, 
%Phys. Rev. B \textbf{85}, 075323 (2012


%\bibitem{urbassek_1997_molecular}   H. M. Urbassek, Nucl. Instrum. Methods Phys. Res. B
%\textbf{122}, 427 (1997).

%\bibitem{nietiadi_2012_sputtering}   M. L. Nietiadi, Y. Rosandi, M. Kopnarski, and H. M. Urbassek, Nucl. Instrum. Methods Phys.
%Res. B \textbf{289}, 97 (2012).

%\bibitem{wucher_2011_kinetic}   A. Wucher and A. Duvenbeck, Nucl. Instrum. Methods Phys. Res. B \textbf{269}, 1655 (2011)

%\bibitem{dft} reference on dft: include in dfg$-$fcse.bib

%\bibitem{bse} reference on bse: include in dfg$-$fcse.bib

%\bibitem{dmft} reference on dmft: include in dfg$-$fcse.bib

%\bibitem{qmc} reference on ground state qmc: include in dfg$-$fcse.bib

%\bibitem{kmc} reference on kmc: include in dfg$-$fcse.bib

%\bibitem{lasse_diss_13} Lasse Rosenthal, Kinetic Monte Carlo Simulations of Metal-Polymer Nanocomposite Formation,  Christian-Albrechts-Universität zu Kiel 2013

%\bibitem{groth_phys_rep_2018} S. Groth, T. Dornheim, and M. Bonitz, Phys. Reports \textbf{744}, 1-86 (2018)

%\bibitem{bo-md} Referenz zu Born-Oppenheimer MD: include in dfg$-$fcse.bib

%\bibitem{runge_gross} E. Runge and E.K.U. Gross,
% "Density-Functional Theory for Time-Dependent Systems". 
% Phys. Rev. Lett. \textbf{52} (12) 997  (1984).

%\bibitem{daw_93} M.S. Daw, S.M. Foiles, and M.I. Baskes, 
%The embedded-atom-method: a review of theory and applications,
%Materials Science Reports \textbf{9}, 251 (1993)

%KMC
%\bibitem{marinov} D. Marinov, C. Teixeira, and V. Guerra,
%Deterministic and Monte Carlo methods for simulation of plasma‐surface interactions,
%Plasma Processes and Polymers \textbf{14}, 1600175 (2016)

%\bibitem{guerra} V. Guerra and J Loureiro,
%Dynamical Monte Carlo simulation of
%surface atomic recombination,
%Plasma Sources Sci. Technol.
%\textbf{13}, 85–94 (2004)


%\bibitem{abraham_jap15} J.W. Abraham, N. Kongsuwan, T. Strunksus, F. Faupel, and M. Bonitz,
%Simulation of Nanocolumn Formation in a Plasma Environment
%J. Appl. Phys. \textbf{117}, 014305 (2015)

%\bibitem{bonitz_cpp12} M. Bonitz, L. Rosenthal, K. Fujioka, V. Zaporojtchenko, F. Faupel, and H. Kersten
%Towards a particle based simulation of complex plasma driven nanocomposite formation
%Contrib. Plasma Phys. \textbf{52} , No. 10, 890-898 (2012)

%\bibitem{fujioka_phd} K. Fujioka,
%\textit{Kinetic Monte Carlo Simulations of Cluster Groth in Magnetron Plasmas}, PhD thesis, Kiel University 2015

%\bibitem{polonski_epjd18} O. Polonskyi, A.M. Ahadi, T. Peter, K. Fujioka, J.W. Abraham, E. Vasiliauskaite, A. Hinz, T. Strunskus, S. Wolf, M. Bonitz, H. Kersten, and F. Faupel, 
%Plasma based formation and deposition of metal and metal oxide nanoparticles using a gas aggregation source,
%Eur. Phys. J. D 72:93 (2018)

%\bibitem{stefanucci-book} G. Stefanucci and R. van Leeuwen

%\bibitem{balzer-book} K. Balzer and M. Bonitz

%% Quantum Statistical Mechanics
%\bibitem{kadanoff62} L.P.~Kadanoff and G.~Baym, \textit{Quantum Statistical Mechanics} (W.A.~Benjamin, Inc.~New York, 1962).

%\bibitem{ojanpera_prb_14} A. Ojanper\"a, A. V. Krasheninnikov, and M. Puska, Phys. Rev.
%B \textbf{89}, 035120 (2014).

%\bibitem{srim}  J. F. Ziegler, M. D. Ziegler, and J. P. Biersack,
%Nucl. Instrum. Meth. B \textbf{268}, 1818 (2010)

%\bibitem{heese_bsc_17} S. Heese, \textit{Dielectric Function of Graphene with Yambo}, Bachelor thesis, Kiel University 2017.

\end{thebibliography}

